Uranus Study Report: KISS

Determining the internal structure of Uranus is a key objective for planetary science. Knowledge of Uranus's bulk composition and the distribution of elements is crucial to understanding its origin and evolutionary path. In addition, Uranus represents a poorly understood class of intermediate-mass planets (intermediate in size between the relatively well studied terrestrial and gas giant planets), which appear to be very common in the Galaxy. As a result, a better characterization of Uranus will also help us to better understand exoplanets in this mass and size regime. Recognizing the importance of Uranus, a Keck Institute for Space Studies (KISS) workshop was held in September 2023 to investigate how we can improve our knowledge of Uranus's internal structure in the context of a future Uranus mission that includes an orbiter and a probe. The scientific goals and objectives of the recently released Planetary Science and Astrobiology Decadal Survey were taken as our starting point. We reviewed our current knowledge of Uranus's interior and identified measurement and other mission requirements for a future Uranus spacecraft, providing more detail than was possible in the Decadal Survey's mission study and including new insights into the measurements to be made. We also identified important knowledge gaps to be closed with Earth-based efforts in the near term that will help guide the design of the mission and interpret the data returned.

==> sections/boilerplate.tex <==
\newpage
\section{boilerplate}\label{sec:boilerplate}

\vfil

Study Report prepared for the W. M. Keck Institute for Space Studies (KISS)\\

Team Leads: Mark Hofstadter, Ravit Helled, and David Stevenson\\

The research was carried out in part at the Jet Propulsion Laboratory, California Institute of Technology, under a contract with the National Aeronautics and Space Administration (80NM0018D0004).\\

Pre-Decisional Information — For Planning and Discussion Purposes Only\\

DOI:  TBD\\



Director: Prof. Bethany Ehlmann
Executive Director: Harriet Brettle
Editing and Formatting: Jessica Law
Cover Image: Keck Institute for Space Studies /Chuck Carter
© 2023. All rights reserved.


==> sections/subsections/atmospheric_dynamics.tex <==
%\subsection{Atmospheric dynamics?}\label{sec:atmospheric_dynamics}
%TBD.. 
%Potential outreach camera (optical \& Doppler) to engage the general public (zonal winds, storms, and swirls). Optical may not be enough in providing context due to hazes.


==> sections/subsections/material_properties.tex <==
\section{Material Properties (Equation of State and Transport Properties}

Our understanding of planet interiors has always involved three essential ingredients: The planetary data (e.g., gravity), the theoretical framework (e.g., the equation of hydrostatic equilibrium), and the material properties of the likely constituents (e.g., the pressure-density relationship determined by laboratory measurement, aided by condensed matter theory). For example, we infer the presence of elements other than iron in Earth's core by determining the extent to which the data-driven determination of the density at a known pressure (provided by hydrostatic equilibrium) differs from the laboratory and theoretical data we have for pure iron. 

For Uranus, as discussed above, we would like to know its compositional and thermal structure, the way heat escapes, and the location and means whereby the magnetic field is created. Even if one had a density profile (from gravity and other measurements) we would not know the composition in general, even if we knew the \textit{equation of state (EoS)} of relevant constituents and thermal structure. This is different from terrestrial and giant planet experience. The main reason is ambiguity: A planet such as Uranus has three components of roughly comparable importance. You can get a specified density by a range of mixtures of these components, for example a mixture of rock and gas can have similar density (and rather similar compressibility) to pure ice. The problem is less central to an understanding of Jupiter and Saturn because they are dominated by a hydrogen-helium component, and the problem does not exist for terrestrial planets where one has two immiscible components (the mantle and core) each with limited compositional variability. The problem is further compounded by the uncertainty in temperature structure: A large increase in temperature can give the same density as a decrease in ice relative to rock for example. The temperature ambiguity is largely absent in terrestrial planets because of the formation of nearly homogeneous layers, each of which might be almost isentropic.

This ambiguity diminishes the value of knowing precise equations of state (EoS, the function $P(\rho,T)$ where $P$ is pressure, $\rho$ is density and $T$ is temperature) but enhances the importance of knowing phase relationships (especially the properties of mixtures), melting curves, and non EoS issues such as the formation and evolution. The ambiguity can only be diminished or eliminated by considering other issues: How was the planet built? How can we create the homogeneous layer that is probably needed to allow generation of magnetic field? How do we explain the heat flow? How can we reconcile interior models with the observable atmospheric composition? This section concentrates on a narrower issue: To what extent does it help to have better knowledge of the EoS of relevant constituents, the phase diagrams, and the microscopic transport properties (electrical conductivity, viscosity, and diffusivity)? These considerations point to a knowledge gap that should be at least partly filled through laboratory and theoretical work, preferably prior to a planetary mission.

\subsection{The EoS}

A standard approximation is \textit{volume additivity}. This estimates the density for a known mixture of pure constituents, each of which has a known equation of state. It is desirable to have experiments and theoretical tests of this assumption, although experience to date suggests that it is a good enough approximation in most cases\footnote{It is easy to think of important possible counterexamples, however. They arise when the end member state is a different phase from the mixture state. An example would be where ``rock" is present as a vapor (or supercritical fluid) when mixed with hydrogen, say, whereas the pure rock phase at the same P and T is a dense fluid or solid.} 

One way to appreciate the experimental or theoretical accuracy required is to ask the following: By how much would I get the wrong mass ratio of rock to ice in a mixture if I got the density of an end member (e.g., ice) wrong by x$\%$?. Since rock is typically 2 to 3 times more dense than ice, the answer is also +x$\%$  within a factor of 2, assuming volume additivity and comparable amounts of ice and rock. (The plus sign means that an increase in the estimated density of ice requires an increase in the amount of ice in the mixture.) Typically, we are interested in this issue at the level of 10$\%$ (with the caveat that we don't know exactly what ``ice" means given the uncertainty in the C/O ratio and the speciation of carbon). This suggests that the current understanding of end member densities at a given pressure (typically several percent or less) might be adequate. 

\subsection{Other Thermodynamic Variables}
 
The EoS is actually a derivative property of the more fundamental Gibbs or Helmholtz free energy. Fortunately, Maxwell provided interrelationships among the relevant variables, reducing the range of possibilities. An important parameter is $\gamma \equiv (\partial \ell nT/\partial \ell n\rho)_S$, often called the Gruneisen parameter. Specific heat is also important though generally less uncertain (simply by counting the available degrees of freedom), though very different for hydrogen than for ice or rock. Compressibility comes from the EoS. The remaining parameter $\alpha$ , the coefficient of thermal expansion, can then be obtained from the Maxwell relations (or the appropriate derivatives of the free energy). All of these must be known in order to compute a model of Uranus thermal structure and evolution. The most challenging (and often most difficult) is the $\gamma$ both for end members and for mixtures. It is needed to assess the temperature gradient and the possibility of convection. The need to have these parameters as well as EoS points to the desirability of a free energy model as the starting point , guided by experiment and theory. Of course, the form (phase or speciation) the material takes becomes most important and is considered next.

\subsection{The Phase Diagrams}

There are two main issues with the relevant phase diagrams: What is the melting curve (more precisely, the liquidus and solidus) for some assumed mean composition and what are the solubilities of constituents (the extent to which constituents can mix down to the atomic level)? This also requires an understanding of speciation; that is, what form does carbon take, for example. (Candidates include methane, heavier hydrocarbons, carbon atoms in a soup dominated by hydrogen, diamond, oxidized as in CO, or some as yet undiscovered alloy.) These two issues of partial solidification and mixing are likely to be interconnected because solid phases are usually lower entropy phases with specific stoichiometries (integer ratios of relevant atoms, as in $H_2O$). By the Gibbs phase rule a coexisting liquid is likely to have a different composition and may be entropically favorable because it lacks a required stoichiometry . (An example is the iron -sulfur system, which has a low solidus at low pressure because the coexisting solid lacks the benefit of the mixing entropy arising from sulfur in the coexisting liquid. Water-ammonia is conceptually similar.) Solid phases in Uranus might also be less likely because the temperature gradient might be higher than in adiabatic models, but still merit some attention because of our current ignorance.

It is not known whether the three components (gas, ice, and rock) mix in all proportions under Uranus conditions. It is likely at deep interior conditions, at sufficiently high T, because then the entropic benefit of mixing outweighs any energy benefit from having pure phases. Certainly mixing is not present at sufficiently low temperature and pressure, near or within the atmosphere. In the standard picture, water clouds form below the observable atmosphere but the base of those clouds at still greater depth\footnote{ defined as the place where the vapor pressure of water at that T divided by the total pressure equals the mixing ratio of water to hydrogen, roughly} is not known because we do not know the mixing ratio of water to hydrogen (it is likely not the same as the ratio of water to hydrogen averaged over the entire planet nor is it necessarily similar to the atmospheric ratio of methane to hydrogen ,despite the similar solar system abundances of C and O).

With these points in mind, here is a partial list of the likely important systems to consider in experiments and theoretical studies, needed to support a Uranus mission:

\textit{1. Superionic ice and its possible alloys or analogues.}

Pure superionic ice is of interest because its high entropy implies (by Clausius-Clapeyron) that it has a large increase of freezing point with pressure, increasing the likelihood that it will be encountered within Uranus. Since the material from which it might form is unlikely to be pure $H_2O$, it is important to understand how other elements are incorporated or excluded from this compound, and the extent to which other superionic materials might be present. Its transport properties are also of interest and are considered below.

\textit{2. Water-hydrogen (more generally H-O)}

Water is slightly ionic at low pressure and increasingly so as pressure increases. Hydrogen remains almost insulating until pressures approaching a Megabar, even for temperatures of a few thousand degrees. Not surprisingly, these two constituents can unmix at quite high temperatures by Uranus standard (as much as a few thousand degrees), provided the pressure is sufficiently high. Some lab data at lower pressure suggest this, though more data are needed at multi GPa pressures. As hydrogen becomes more able to give up electrons (not necessarily metallize), a mixture might be preferred, so it is also important to understand the likely solubility at very high (Megabar) pressures since we cannot exclude the presence of hydrogen deep down (even though many Uranus models assume it). Different ratios of H to O must also be considered as alternatives to ice and molecular hydrogen.

\textit{3. Carbon and its Compounds}

Carbon is only modestly less abundant than oxygen by mass. Moreover, it is usually very different in its chemical and bonding behavior. At low pressure but high hydrogen partial pressure, methane is the expected main carrier of carbon within the outer regions of Uranus and is present in the atmosphere at a level far higher than the C/H primordial solar value. However, methane has limited solubility in water at depth, raising the possibility that it has partitioned between atmosphere and deep interior. Equally important, methane is known to decompose at high pressure and temperature, forming heavier hydrocarbons and eventually even diamond. The latter phase cannot be excluded as relevant for Uranus at present, but entropy considerations (the benefit of mixing) suggest many other possibilities.

\textit{4. Nitrogen and its Compounds}

Nitrogen is less abundant than oxygen by about a factor of 6, assuming primordial solar system abundances. For this reason it might be less important. Even so, it is of value to understand its disposition. It might also be diagnostic of phase transitions within the planet. For example, nitrogen (as ammonia) is far more soluble than methane in water. If water has a high pressure (somewhat ionic) phase that separates at depth, then it might partition ammonia downward. This is of interest because ammonia is observed (though apparently depleted) in the Uranus atmosphere.

\textit{5. Rock and Ice (e.g., Water and Silicates}

Rock and ice are quite possibly the most important ``binary" system to consider at high pressure. Current evidence suggests that it is indeed an intimate mixture at the relevant T and P deep within Uranus and fails to separate into two components (as it undoubtedly does in Ganymede, for example, where the pressure and temperature are far lower). This system needs to be better understood: What is the liquidus and solidus?

\subsection{Microscopic Transport Processes}

These are diffusive processes (thermal diffusion, atomic or molecular interdiffusion, viscosity, magnetic diffusivity or equivalently electrical conductivity). They range enormously, though in most cases the required accuracy is far less than for thermodynamic variables. Three specific issues are highlighted here:

\textit{1. Magnetic Diffusivity}

Magnetic diffusivity is likely to be the most important, since it is needed to understand the magnetic field observations, specifically the ability to operate a dynamo. The requirement of an adequate magnetic Reynolds number typically can be met at quite modest electrical conductivity (i.e., without a metal). Traditionally, the field that Uranus possesses has been attributed to a material that is mostly water and has protonic conduction. However, this is not known and a small ``free" electron contribution could easily be of importance if the temperature is high enough. Guided by the phase diagram considerations above, both theoretical and experimental work is needed on the electrical conductivity of candidate Uranus materials,

\textit{1. Thermal Diffusivity}

The measured heat flow from the Uranus interior is sufficiently low that the possibility of conductive heat transport cannot be excluded. As an analogy, the heat flux from Earth's core (which might not be more than a factor of a few smaller than the heat flux deep within Uranus) is thought to be comparable to what is carried by electronic conduction along an adiabatic temperature gradient. Thermal diffusivity is also potentially relevant in any model that involves a large number of boundary layers (e.g., double diffusive convection) since the properties of those layers depends on microscopic heat transport.

\textit{3. Viscosity and Interdiffusion}

Boundary layers (as in double diffusive convection, where there are many ``steps" or layers) also depend on the value of viscosity and diffusivity of atoms or molecules. 

Viscosity (more precisely, rheology) is also of interest for any solid phase, since it affects the tidal response and the ability to convect heat.

\end{section}
